Evaluating Saliency Methods for Neural Language Models

Saliency methods are widely used to interpret neural network predictions, but different variants of saliency methods often disagree even on the interpretations of the same prediction made by the same model. In these cases, how do we identify when are these interpretations trustworthy enough to be used in analyses? To address this question, we conduct a comprehensive and quantitative evaluation of saliency methods on a fundamental category of NLP models: neural language models. We evaluate the quality of prediction interpretations from two perspectives that each represents a desirable property of these interpretations: plausibility and faithfulness. Our evaluation is conducted on four different datasets constructed from the existing human annotation of syntactic and semantic agreements, on both sentence-level and document-level. Through our evaluation, we identified various ways saliency methods could yield interpretations of low quality. We recommend that future work deploying such methods to neural language models should carefully validate their interpretations before drawing insights.

==> source/interpretation.tex <==
\section{Methods for Interpretation}

\citet{DBLP:journals/cacm/Lipton18} describes two different paths for improving interpretability: transparent model architecture, and post-hoc interpretation.

% \emph{Transparent model architectures} allow humans to easily understand their decision-making procedure, thus making their predictions interpretable.
\textbf{Transparent model architectures} generate predictions with interpretable behaviors, but often perform worse compare to their less interpretable counterparts or require lots of expertise to develop.
The most widely used NLP model that was once considered to be transparent is attention \cite{DBLP:journals/corr/BahdanauCB14,DBLP:conf/iclr/SeoKFH17,DBLP:conf/iclr/XiongZS17,DBLP:conf/nips/VaswaniSPUJGKP17}.
However, this has been recently challenged by several analyses \cite{jain-wallace-2019-attention,serrano-smith-2019-attention,wiegreffe-pinter-2019-attention,DBLP:journals/corr/abs-1909-11218,vig-belinkov-2019-analyzing}, and the current consensus is that for many applications, explanations from attention weights are of rather low quality \cite{wiegreffe-pinter-2019-attention,li-etal-2019-word,ding-etal-2019-saliency,vig-belinkov-2019-analyzing}.

\textbf{Post-hoc interpretation} aims to reach a good interpretation of a specific model decision after-the-fact.
This is usually done by measuring the importance of an input feature by the impact on the prediction score when it is perturbed, which is also often referred to as \emph{saliency}.
Such method is traditionally more prevalent in the field of computer vision \cite{DBLP:journals/corr/SimonyanVZ13,DBLP:conf/cvpr/JiangWYWZL13,DBLP:conf/cvpr/LiY15,DBLP:journals/corr/PanWJ15,DBLP:conf/cvpr/OhBKAFS17}, but is also gaining popularities in NLP recently \cite{li-etal-2016-visualizing,DBLP:journals/corr/LiMJ16a,arras-etal-2016-explaining,arras-etal-2017-explaining,mudrakarta-etal-2018-model,ding-etal-2019-saliency}.
The beauty of this method is that it is model-agnostic but yet gives insights about the model behavior by using the original model to measure the feature importance.
Note that one could also build another model that is specifically trained to generate certain interpretations \cite[e.g., LIME,][]{ribeiro-etal-2016-trust}, but they only work for classification but not sequence generation \cite{poerner-etal-2018-evaluating}.

The rest of this section will briefly introduce the various post-hoc interpretation methods we will analyze in this paper.
We will first introduce the general mathematical formulation of saliency, and then discuss the NLP-specific concern of how to compute saliency for words.
% Although there are some previous work \cite{poerner-etal-2018-evaluating,arras-etal-2019-evaluating} that conducted comprehensive qualitative analysis on the viability of these methods on recurrent architectures, these analysis generally stops at single-layer recurrent models and no analysis has been conducted for Transformer models.

\subsection{General Saliency} \label{sec:general-saliency}

Consider the general case of a classifier $\vec{f}: \R^d\rightarrow\R^{\mid\mathcal{C}\mid}$ that produces a output distribution $\vec{f}(\vec{x})$ over classes $\mathcal{C}$ from an input feature vector $\vec{x}$.
Given a specific input example $\vec{x_0}$, the saliency vector $\vec{\Psi}$ \cite{DBLP:journals/corr/SimonyanVZ13} of $\vec{x_0}$ for a specific class prediction $c\in\mathcal{C}$ is defined by:
\begin{align}
    \vec{\Psi}(\vec{x_0}, c, \vec{f}) = \dfrac{\partial f_c(\vec{x})}{\partial \vec{x}} \bigg|_{\vec{x_0}}
\end{align}
where $\vec{\Psi}, \vec{x_0}\in\R^d$.
To distinguish this method from its later variants that generate superior interpretations, we will refer to this method  as \textbf{vanilla (V)} saliency for the rest of the paper.
% We now switch to the introduction of these variants.
% \item \textbf{Guided Back-propagation}: \citet{DBLP:journals/corr/SpringenbergDBR14} proposed to modify the back-propagation procedure for the ReLU function to only pass over the positive gradients propagated from the succeeding node in the computation graph. This will make the back-propagation procedure of the ReLU function guided by the information flowing both from preceding and succeeding nodes.

\vspace{0.2cm}
\noindent \textbf{Integrated Gradients (IG)}\quad  \citet{DBLP:conf/icml/SundararajanTY17} proposed to compute feature importance by computing a line integral of the vanilla saliency from a ``baseline'' point $\vec{x_b}$ to the input $\vec{x_0}$ in the feature space.
% The methods mentioned above mostly concerns about what would be responsible for perturbation of the model output in the neighborhood of $\vec{x_0}$.
% Different from the others, \citet{DBLP:conf/icml/SundararajanTY17} proposed to decompose the output value of the model to each input feature according to their importance. This is computed with a integral from a "baseline" to the original input $\vec{x_0}$:
\begin{align}
\vec{\Psi}_{IG}&(\vec{x_0}, c, \vec{f}) \notag = (\vec{x_0} - \vec{x_b})\odot \\ &\int_{\alpha = 0}^1 \vec{\Psi}(\vec{x_b} + \alpha(\vec{x_0} - \vec{x_b}), c, \vec{f})\,\text{d}\alpha
\end{align}
This feature importance measure has been shown to have several good axiomatic properties. In practice, the integration is evaluated by dividing the line between $\vec{x_b}$ and $\vec{x_0}$ into $N$ steps and summing up the attribution of each slice. % Note that $\vec{x_b}$ should be close to 0 for the saliency scores to be interpreted as a decomposition of the output score.

\vspace{0.2cm}
\noindent \textbf{SmoothGrad (SG)}\quad \citet{DBLP:journals/corr/SmilkovTKVW17} proposed to reduce the noise in saliency scores by constructing several corrupted instances of the original input by adding Gaussian noise, followed by averaging the scores.
\begin{align}
\vec{\Psi}_{SG}(\vec{x_0}, c, \vec{f}) &= \dfrac{1}{N}\sum_{i=1}^N \vec{\Psi}(\vec{x_0} + \Delta \vec{x}, c, \vec{f}) \notag\\
\Delta \vec{x} &\sim \mathcal{N}(\vec{0}, \sigma^2\vec{I}) \label{fm:vanilla-saliency}
\end{align}
% Note that this is a general smoothing technique that can be used on top of any saliency methods, including both vanilla saliency and integrated gradients mentioned above.

\subsection{Word Saliency} \label{sec:word-saliency}

Up to now, we have discussed the formulation of saliency in the context of a classifier, where we simply compute one saliency score for each input feature.
This works out of the box for computer vision, where each input feature is simply an individual pixel.
However, for most NLP problems, each input word may correspond to a word vector.
In this case, it is straight-forward to compute saliency scores for each dimension of the word vector, but for most NLP applications, people are more concerned with word-level importance measures than the neuron-level ones.
% Unfortunately, there is no clear consensus on how per-dimension saliency scores should be composed to form the saliency for a word.
As there is no clear consensus, we also compare with two previously proposed composition scheme for this problem.

% Huda: "YOu should save this paragraph for your thesis."
% Up to now, we have discussed the formulation of saliency in the context of a classifier, where we simply compute one saliency score for each input feature.
% This works out of the box for computer vision, where each input feature is simply an individual pixel.
% However, for most NLP problems, each input word may correspond to a word vector.
% In this case, it is straight-forward to compute saliency scores for each dimension of the word vector, but for most NLP applications, people are more concerned about word-level importance measures then the neuron-level ones.
% Unfortunately, there is no clear consensus on how per-dimension saliency scores should be composed to form the saliency for a word.
% In this paper, we also compare with two previously proposed composition scheme for this problem.

Consider, again, the case of a classifier with natural language input. Suppose we have obtained saliency scores for each dimension of the word embedding $\vec{e}_w$ corresponding to an input word $w$, denoted as $\vec{\Psi}_w$.
Noting that $\vec{\Psi}_w$ would be a vector, we define a scalar score $\psi_w$ for word $w$ that is composed from $\vec{\Psi}_w$.
The schemes are as follows.

\vspace{0.2cm}
\noindent \textbf{Vector Norm (VN)}\quad \citet{li-etal-2016-visualizing} proposed to measure word saliency by computing a scaled L1-norm of the $d$-dimensional gradient vector: $$\psi_w = \frac{1}{d} \left\| \vec{\Psi}_w \right\|_1$$

Similar vector norm formulation has been adopted by previous NLP interpretability studies \cite{arras-etal-2016-explaining,arras-etal-2017-explaining}, including a toolkit for interpreting NLP models \cite{Wallace2019AllenNLP}.

\vspace{0.2cm}
\noindent \textbf{Gradient $\cdot$ Input (GI)}\footnote{Note that this approach should not be mistaken with Gradient $\odot$ Input \cite{DBLP:journals/corr/ShrikumarGSK16} in the context of computer vision, which conducts element-wise product instead of dot product.}\quad
\citet{DBLP:journals/corr/DenilDF14} compute the saliency score of a sentence by taking dot product of the sentence embedding $\vec{e}_w$ and its saliency score. % used this scheme on sentence embedding to extract salient sentences, and motivated it by
\citet{mudrakarta-etal-2018-model,DBLP:conf/iclr/MurdochLY18,ding-etal-2019-saliency} also adopted the same scheme and extended it to word embedding.
$$\psi_w = \vec{e}^T_w \vec{\Psi}_w$$
Multiple studies \cite{DBLP:journals/corr/DenilDF14,ding-etal-2019-saliency} motivated this scheme by showing it is equivalent to taking gradient with regard to the 1 in the one-hot vector for the look-up operation.
% In this composition scheme, the word saliency score is computed by taking dot product of $\vec{e}_w$ and its saliency score: $$\psi_w = \vec{e}^T_w \vec{\Psi}_w$$

% This approach dates back to study by \citet{DBLP:journals/corr/ShrikumarGSK16} for computer vision, and is used in NLP by \citet{mudrakarta-etal-2018-model,ding-etal-2019-saliency}. The formulation is as follows: $$\psi_w = \vec{e}^T_w \vec{\Psi}_w$$ where $\vec{e}_w$ is the word embedding corresponding to word $w$.

\subsection{Other Methods}

There are lots of other post-hoc interpretation methods that were investigated in previous literature such as \citet{poerner-etal-2018-evaluating,arras-etal-2019-evaluating} but we choose to leave out for the analysis in this paper.
While \citet{poerner-etal-2018-evaluating,arras-etal-2019-evaluating} both show that DeepLIFT~\cite{DBLP:conf/icml/ShrikumarGK17} and LRP~\cite{bach2015pixel} tend to generate the optimal interpretations, they also both require manually re-defining back-propagation rules for each layer in the network.
This might be feasible for the simple recurrent models as used in \citet{poerner-etal-2018-evaluating,arras-etal-2019-evaluating}, but is impractical for real-world models, especially architectures that have not been previously explored for these methods, such as Transformer.
% Hence, we leave them for future work and focus on the architecture-invariant Integrated Gradients \cite{DBLP:conf/icml/SundararajanTY17} method, which was also recommended by \citet{poerner-etal-2018-evaluating}.
We also leave out contextual decomposition \cite{DBLP:conf/iclr/MurdochLY18} because it is only designed for LSTM.
Finally, we leave out occulusion-based methods \cite{DBLP:conf/eccv/ZeilerF14,DBLP:journals/corr/LiMJ16a,li-etal-2019-word} because (1) they were shown to perform inconsistently in both \citet{poerner-etal-2018-evaluating,arras-etal-2019-evaluating}, and (2) they are not viable for long document-level contexts because separate forward passes needs to be computed for each input word.


==> source/intro_acl2020.tex <==
\section{Introduction}

% As a deep learning architecture, Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} has recently become popular for various tasks such as neural machine translation~\cite{DBLP:conf/nips/VaswaniSPUJGKP17}, language modeling~\cite{DBLP:conf/iclr/BaevskiA19,dai-etal-2019-transformer} and pre-training representations for downstream tasks~\cite{radford2019language,devlin-etal-2019-bert}.
Neural language models, including RNN-based neural language models~\cite{DBLP:conf/interspeech/MikolovKBCK10} and their variants~\cite{DBLP:conf/iclr/MerityKS18,DBLP:conf/iclr/0002MXS17}, and later Transformer language models~\cite{DBLP:conf/iclr/BaevskiA19,dai-etal-2019-transformer}, have been dominating the state-of-the-art of language modeling task.
Because of their impressive ability to acquire linguistic knowledge from practically unlimited amount of data, they have also been used as a pre-training step for a wide range of NLP tasks~\cite{peters-etal-2018-deep,radford2019language,devlin-etal-2019-bert}.
However, a general complaint is that they lack interpretability.
Previous efforts to improve neural language model interpretability mainly focused on representation probing \cite[\textit{inter alia}]{DBLP:conf/acl/TenneyDP19} and attention analysis \cite{vig-belinkov-2019-analyzing}.
The former only provide limited understanding of the model decision mechanism, and the latter is only applicable for Transformer and requires a painstaking process of selecting the right attention head.
% Previous work~\cite{ding-etal-2019-saliency} has shown that in the context of neural machine translation, the prediction from Transformer models is less interpretable compared to other common architectures such as LSTM and CNN.
% This raises the question whether the superior of Transformer model comes at an expense of less interpretable behaviors.

\setlength{\fboxsep}{2pt}
\begin{table}[t]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{p{0.56\textwidth}}

\toprule
{\bf PTB} \quad
{\tt \colorbox{bananamania!21.16068315382694!white}{(U.S.}
\colorbox{applegreen!6.976635665770241!white}{Trade}
\colorbox{bananamania!11.646363110441373!white}{Representative}
\colorbox{bananamania!8.149284362292839!white}{Carla}
\colorbox{bananamania!3.419342434429997!white}{Hills)}
\colorbox{bananamania!15.272963526440947!white}{said}
\colorbox{applegreen!5.767504311209829!white}{the}
\colorbox{applegreen!3.7131208951511354!white}{first}
\colorbox{bananamania!1.8217670400367418!white}{dispute-settlement}
\colorbox{bananamania!3.4057709333970365!white}{(panel)}
\colorbox{applegreen!3.6528102693661593!white}{set}
\colorbox{applegreen!5.83930272012406!white}{up}
\colorbox{applegreen!17.8511069694809!white}{under}
\colorbox{applegreen!8.3255954255329!white}{the}
\colorbox{bananamania!1.308298119380497!white}{U.S.-Canadian}
\colorbox{applegreen!12.625602443313824!white}{``}
\colorbox{bananamania!4.4480144556232935!white}{free}
\colorbox{applegreen!5.422068372289055!white}{(trade)}
\colorbox{bananamania!0.5897984027435099!white}{''}
\colorbox{applegreen!15.901601612440736!white}{(agreement)}
\colorbox{applegreen!12.655945799807848!white}{has}
\colorbox{applegreen!12.022714234352058!white}{ruled}
\colorbox{applegreen!34.44695613303782!white}{that}
\colorbox{bananamania!0.5579945664227938!white}{(Canada)}
\colorbox{applegreen!15.76725082152275!white}{'s}
\colorbox{applegreen!54.019444079144485!white}{[restrictions]}
\colorbox{bananamania!28.655321287684377!white}{on}
\colorbox{applegreen!100.0!white}{[exports]}
\colorbox{applegreen!3.7675680795128654!white}{of}
\colorbox{applegreen!9.982807819175314!white}{(Pacific}
\colorbox{applegreen!38.423514331756444!white}{salmon)}
\colorbox{bananamania!29.008341808962733!white}{and}
\colorbox{bananamania!59.608387716108446!white}{(herring)}
| PLURAL}
\\\midrule

{\bf Syneval}
{\tt \colorbox{applegreen!17.241609155665046!white}{the}
\colorbox{applegreen!12.68599210446062!white}{[consultant]}
\colorbox{bananamania!22.998325684906334!white}{that}
\colorbox{applegreen!2.2922756993317877!white}{loves}
\colorbox{bananamania!42.2468290198368!white}{the}
\colorbox{bananamania!100.0!white}{(parents)}
| SINGULAR}
\\\midrule

{\bf CoNLL}
{\tt \colorbox{bananamania!22.23870329914711!white}{[Israeli}
\colorbox{bananamania!5.95411997972827!white}{Prime}
\colorbox{applegreen!9.82677284982589!white}{Minister}
\colorbox{bananamania!0.19090535271031644!white}{Ehud}
\colorbox{bananamania!2.8275234066195787!white}{Barak]}
\colorbox{bananamania!7.337541289339324!white}{says}
\colorbox{applegreen!29.84703357129253!white}{[he]}
\colorbox{applegreen!3.598859733494998!white}{is}
\colorbox{bananamania!3.5239570370685693!white}{freezing}
\colorbox{applegreen!0.8378664755702526!white}{tens}
\colorbox{applegreen!3.811363591325725!white}{of}
\colorbox{bananamania!0.8678509029617497!white}{millions}
\colorbox{applegreen!3.224034780844022!white}{of}
\colorbox{bananamania!3.5209368280906594!white}{dollars}
\colorbox{applegreen!4.377595205390724!white}{in}
\colorbox{bananamania!3.653914785335803!white}{tax}
\colorbox{bananamania!3.5822272536612236!white}{payments}
\colorbox{applegreen!0.42086484812532365!white}{to}
\colorbox{applegreen!2.5045683871827173!white}{the}
\colorbox{applegreen!10.106480715250074!white}{Palestinian}
\colorbox{applegreen!1.674910925853686!white}{Authority}
\colorbox{applegreen!21.94343842168209!white}{.}
\colorbox{applegreen!14.56546880946151!white}{[Mr.}
\colorbox{bananamania!7.734577209275528!white}{Barak]}
\colorbox{bananamania!7.938630307705349!white}{says}
\colorbox{applegreen!49.74066937078735!white}{[he]}
\colorbox{applegreen!4.514930768222998!white}{is}
\colorbox{bananamania!0.7932005595827049!white}{withholding}
\colorbox{applegreen!5.552661545400199!white}{the}
\colorbox{applegreen!0.9074348379821188!white}{money}
\colorbox{applegreen!2.1402910006212896!white}{until}
\colorbox{applegreen!5.263565527342066!white}{the}
\colorbox{applegreen!7.033072664466526!white}{Palestinians}
\colorbox{applegreen!4.038979962032707!white}{abide}
\colorbox{applegreen!1.8408821661614025!white}{by}
\colorbox{applegreen!2.7857113564628255!white}{cease}
\colorbox{bananamania!1.9756056656624992!white}{-}
\colorbox{bananamania!2.0194486962642255!white}{fire}
\colorbox{bananamania!4.94053481919297!white}{agreements}
\colorbox{bananamania!35.04097098801201!white}{.}
\colorbox{bananamania!8.47142746525934!white}{Earlier}
\colorbox{applegreen!2.441945840276817!white}{Thursday}
\colorbox{applegreen!7.820459585530447!white}{[Mr.}
\colorbox{bananamania!4.279523735429693!white}{Barak]}
\colorbox{bananamania!4.45592614176193!white}{ruled}
\colorbox{applegreen!5.03750811474739!white}{out}
\colorbox{bananamania!4.4378947969102125!white}{an}
\colorbox{bananamania!5.325400911640722!white}{early}
\colorbox{bananamania!1.5618542376687952!white}{resumption}
\colorbox{bananamania!0.7372805921848148!white}{of}
\colorbox{bananamania!0.050577494696514874!white}{peace}
\colorbox{bananamania!4.184111462225186!white}{talks}
\colorbox{applegreen!3.648809696375419!white}{,}
\colorbox{applegreen!0.74557573100617!white}{even}
\colorbox{bananamania!2.375379682103739!white}{with}
\colorbox{applegreen!4.1475808786642965!white}{the}
\colorbox{applegreen!2.1777816840288926!white}{United}
\colorbox{bananamania!5.944706138804108!white}{States}
\colorbox{applegreen!0.5244119376970888!white}{acting}
\colorbox{applegreen!0.9860935294132758!white}{as}
\colorbox{bananamania!8.110537263250295!white}{intermediary}
\colorbox{bananamania!100.0!white}{.}
\colorbox{bananamania!35.80773342307109!white}{(Eve}
\colorbox{applegreen!9.224652171376126!white}{Conette)}
\colorbox{applegreen!8.053899170525108!white}{reports}
\colorbox{bananamania!14.090324432096125!white}{from}
\colorbox{applegreen!34.75532087059817!white}{Jerusalem}
\colorbox{applegreen!53.00765474350793!white}{.}
\colorbox{bananamania!12.159119141189082!white}{Defending}
\colorbox{applegreen!73.88800712813357!white}{what}
| MALE
} \\\midrule

{\bf Winobias} \quad
{\tt \colorbox{bananamania!38.453172719964634!white}{The}
\colorbox{applegreen!100.0!white}{[bride]}
\colorbox{bananamania!17.781165314642365!white}{examined}
\colorbox{bananamania!29.737045759985314!white}{the}
\colorbox{bananamania!32.20225609955182!white}{(son)}
\colorbox{applegreen!21.327052369358977!white}{for}
\colorbox{applegreen!4.51699784864446!white}{injuries}
\colorbox{bananamania!5.522630817506281!white}{because}
| FEMALE
} \\
\bottomrule

    \end{tabular}
    }
    \caption{Examples of our benchmark tests used to evaluate post-hoc interpretations from language models, with interpretation of the argmax prediction (last all-caps token of each example) from our distilled Transformer language model (Section \ref{sec:distill}). Postive and negative word importance (``saliency'') are marked as {\setlength{\fboxsep}{1pt}\colorbox{applegreen}{green}} and {\setlength{\fboxsep}{1pt}\colorbox{bananamania}{yellow}}, respectively, while cue and attractor words are marked with [] and () (more details in Section \ref{sec:test-formulation}).}
    \label{tab:pitch}
\end{table}

In this paper, we focus on \emph{post-hoc interpretation}, a category of interpretation method that is rarely visited in the context of language modeling, but has been successfully adopted in computer vision.
% We systematically and qualitatively evaluate the viability of post-hoc interpretation methods for Transformer architectures.
These methods generally require less effort to set up, and are often agnostic to model architectures.
Different from several previous work on evaluating interpretation methods, all of our analyses are conducted on state-of-the-art or real-world-scale models.
Our main contributions are:

\begin{itemize}[topsep=1pt] \itemsep -2pt
\item Exemplified in Table \ref{tab:pitch}, we construct four new interpretability benchmark datasets based on exisiting human annotations of syntactic and semantic agreements.
% Not only our benchmark covers agreements within a single sentence, but it also contains more challenging tasks such as gender agreement between the pronoun and its antecedants on the document-level, which is not previously studied in the context of interpretability.
% \sd{is lexical agreement a mere syntactic notion or could also be used in the semantic context?}
\item We propose to use representation probes on top of interpreted models to generate more informative benchmark results.
\item We show that the viability of post-hoc interpretation methods for neural language models depends on multiple factors such as model configurations, post-hoc interpretation methods, and the models' training approach.
\item We show that by taking advantage of knowledge distillation, it is possible to build neural language models with solid task performance and good interpretability at the same time.
% \cite{DBLP:journals/corr/HintonVD15,kim-rush-2016-sequence}
\end{itemize}

==> source/method.arxiv.tex <==
\section{Benchmark}

% The major challenge to design NLP benchmark tests for salience methods is the ambiguity of the ground truth.
% In the context of computer vision, image classification and human-generated pixel-level ground truth constitutes a reliable benchmark, because the input image generally contains a clear, salient object that could be recognized by humans with little ambiguity.
% In constrast, because of the compositional nature of the natural language, it is usually hard to point to a definite part of the input that is responsible for the model output with clear consensus. \shuoyang{probably too sloppy?}

We propose to construct a test with a well-studied sentence-level dependency -- the \textit{subject-verb agreement} in the present tense of English\footnote{In our experiment, we also includ cases of ``was'' and ``were'' to get more examples. They are not present tense verbs but the behavior is very similar.}.
The biggest advantage of this depenedency is that it has a clear ``salient word'' -- the subject -- that is responsible for predicting the morphological number of the verb,
and has been used in various studies~\cite{DBLP:journals/tacl/LinzenDG16,DBLP:conf/emnlp/MarvinL18} as a probe to investigate how neural network models make predictions.
Moreover, with this choice, our test can be conducted with a language model, which is one of the most basic NLP tasks.
It is also very versatile in terms of the neural architectures that could be used, as previous work has attempted many different variants including RNN~\cite{DBLP:conf/interspeech/MikolovKBCK10}, CNN~\cite{pham-etal-2016-convolutional}, and self-attention~\cite{DBLP:journals/corr/abs-1808-04444}.

Formally, the test is described as follows:
\begin{defi}
Suppose we have the prefix of a sentence immediately preceding a verb (referred to as ``prefix''), the subject of that verb (referred to as ``subject'') and an alternative noun in the sentence that has a different morphological number from the subject (referred to as ``attractor''). In that case, the test will ask one of the following questions depending on the prediction distribution for the word following the prefix, generated by the language model:
\begin{itemize}[leftmargin=*] \itemsep -2pt
\item If the language model prefers the verb with the same morphological case as the subject (\textit{positive case}), is the salience of the subject higher than the attractor when predicting the singular verb?
\item If the language model prefers the verb with the different morphological case as the subject (\textit{negative case}), is the salience of the attractor higher than the subject when predicting the plural verb?
\end{itemize}
An interpretation passes the test if it gives affirmative answer to the corresponding question.
\end{defi}

Here is the intuition behind the test: syntactically, a human would solely resort to the subject to determine the morphological number of a verb, instead of other nouns in the sentence, e.g. an object or the subject of an intervening clause.
If the model made the correct prediction but the interpretation does not conform to this human intuition, it is certain that either the model is relying on the wrong evidence to make the prediction, or the salience method is not making a correct interpretation.
Because the salience method does not intervene with the model's prediction procedure, neither the prediction nor the ``evidence of prediction'' should change with the choice of the salience method.
Hence, if we hold the language model constant, we'll be able to evaluate the performance of the salience method by comparing the fraction of instances that passes the test with different salience methods.

Note that we made an implicit assumption in the argument above: the language model relies only on the syntactic relations to determine the next word.
This is not true, because semantic relation also plays a large role in this prediction.
Hence, we follow \citet{DBLP:journals/tacl/LinzenDG16} and strip away the semantics of the verb prediction by substituting all the present-tense verb as well as past-tense copulas in the corpus with their POS tag, VBZ (singular) or VBP (plural)\footnote{We ignore the tense and use the same tag for past-tense copulas as well.}.
% \footnote{One may also argue that the model may have a tendancy to look at closer words because they are necessary to decide when does the verb occur. We will empirically show that this does not have much influence in the interpretation generated.}
In the analysis part, we will compare results in both cases to show how much semantic relations influence the interpretation.

Below is an example of the test described above. 

\vspace{0.2cm}
\hspace{-0.45cm}
\begin{tabular}{@{}llll@{}}
\textbf{prefix} & \multicolumn{3}{l}{\textit{\begin{tabular}[c]{@{}l@{}}But New York state , which VBZ see-\\king solutions to its prison cell shortage ,\end{tabular}}} \\
\textbf{subject} & \textit{state\hspace{1cm}} & \textbf{attractor} & \textit{solutions} \\
\end{tabular}
\vspace{0.2cm}

Depending on whether the language model prefers VBZ or VBP for the next word, the intterpretation will be tested with different questions as mentioned above.


==> source/preliminaries.tex <==
\section{Preliminaries}

In this section, we clarify certain concepts regarding our scope of the investigation.

\subsection{Saliency Methods}

According to \citet{DBLP:journals/cacm/Lipton18}, there are two different paths for modeling interpretability.
One of them, which aims for building \emph{transparent model architectures} that allow humans to easily understand their decision-making procedure, can be examplified by the use of attention mechanisms in various NLP tasks \cite[\textit{inter alia}]{DBLP:journals/corr/BahdanauCB14,DBLP:conf/nips/VaswaniSPUJGKP17,DBLP:conf/iclr/SeoKFH17}.
There has been extensive discussion on whether attention could be treated as an explanation for the prediction made by such models \cite{jain-wallace-2019-attention,serrano-smith-2019-attention,wiegreffe-pinter-2019-attention}.
The other, referred to as \emph{post-hoc interpretability}, aims to reach a good interpretation of a specific model decision after-the-fact, with or without relying on the original decision mechanism of the model.
In this paper, we focus on \emph{saliency methods}, which falls into the latter.

Saliency methods measure the importance of an input feature by its impact on the model prediction score -- more specifically, originally by utilizing the gradients of the prediction score on input features \cite{DBLP:journals/corr/SimonyanVZ13}.
Since then, various improvements over this method have been proposed to counteract noisy gradients \cite{DBLP:journals/corr/SmilkovTKVW17}, to enforce axiomity \cite{DBLP:conf/icml/SundararajanTY17}, to isolate certain input patterns \cite{DBLP:journals/corr/SpringenbergDBR14} or to define better backward attribution rules \cite{bach2015pixel}.
% These methods are traditionally more prevalent in the field of computer vision \cite{DBLP:journals/corr/SimonyanVZ13,DBLP:conf/cvpr/JiangWYWZL13,DBLP:conf/cvpr/LiY15,DBLP:journals/corr/PanWJ15,DBLP:conf/cvpr/OhBKAFS17}, but is also gaining popularities in NLP recently \cite{li-etal-2016-visualizing,DBLP:journals/corr/LiMJ16a,arras-etal-2016-explaining,arras-etal-2017-explaining,mudrakarta-etal-2018-model,ding-etal-2019-saliency}, and sometimes used as a proxy for ground-truth interpretation for evaluating interpretation methods that do not fall into this category \cite{jain-wallace-2019-attention}.
The major strength of these methods is that their definitions are model-agnostic but yet give insights about the model behavior when measuring feature importance.
However, several papers also pointed out that saliency methods are subject to implausible and/or unfaithful interpretations under certain settings for computer vision models \cite{DBLP:conf/nips/AdebayoGMGHK18,DBLP:series/lncs/KindermansHAASDEK19,DBLP:conf/nips/HeoJM19,DBLP:conf/aaai/GhorbaniAZ19,yeh2019fidelity}.
Similar evaluations on neural language models were previously done in \citet{poerner-etal-2018-evaluating,arras-etal-2019-evaluating}, but largely constrained to small-scale models or artificial tasks.

% \citet{DBLP:journals/cacm/Lipton18} describes two different paths for improving interpretability: transparent model architecture, and post-hoc interpretation.

% \emph{Transparent model architectures} allow humans to easily understand their decision-making procedure, thus making their predictions interpretable.
% \textbf{Transparent model architectures} generate predictions with interpretable behaviors, but often perform worse compare to their less interpretable counterparts or require lots of expertise to develop.
% The most widely used NLP model that was once considered to be transparent is attention \cite{DBLP:journals/corr/BahdanauCB14,DBLP:conf/iclr/SeoKFH17,DBLP:conf/iclr/XiongZS17,DBLP:conf/nips/VaswaniSPUJGKP17}.
% However, this has been recently challenged by several analyses, and the current consensus is that for many applications, explanations from attention weights are of rather low quality \cite{jain-wallace-2019-attention,serrano-smith-2019-attention,wiegreffe-pinter-2019-attention,li-etal-2019-word,ding-etal-2019-saliency,DBLP:journals/corr/abs-1909-11218,vig-belinkov-2019-analyzing}.
%
% \textbf{Post-hoc interpretation} aims to reach a good interpretation of a specific model decision after-the-fact.
% Such method is traditionally more prevalent in the field of computer vision \cite{DBLP:journals/corr/SimonyanVZ13,DBLP:conf/cvpr/JiangWYWZL13,DBLP:conf/cvpr/LiY15,DBLP:journals/corr/PanWJ15,DBLP:conf/cvpr/OhBKAFS17}, but is also gaining popularities in NLP recently \cite{li-etal-2016-visualizing,DBLP:journals/corr/LiMJ16a,arras-etal-2016-explaining,arras-etal-2017-explaining,mudrakarta-etal-2018-model,ding-etal-2019-saliency}.
% This is usually done by measuring the importance of an input feature by the impact on the prediction score when it is perturbed, which is also often referred to as \emph{saliency}.
%
% The beauty of this method is that it is model-agnostic but yet gives insights about the model behavior by using the original model to measure the feature importance.
% Note that one could also build another model that is specifically trained to generate certain interpretations \cite[e.g., LIME,][]{ribeiro-etal-2016-trust}, but they only work for classification but not sequence generation \cite{poerner-etal-2018-evaluating}.

% Apart from that, probing... ?

\subsection{Plausibility and Faithfulness}

Following the proposal in \citet{DBLP:journals/corr/abs-2004-03685}, we conduct our investigation from two perspectives: \emph{plausibility} and \emph{faithfulness}.
We now briefly explain what these two perspectives mean within the scope of our investigation.

As saliency methods generate a distribution of importance over the input features, a perfect interpretation should ideally reflect the importance of each input feature under the model's reasoning process to reach the decision.
However, such a reasoning process is more of a concept than a practically attainable ground truth for evaluation.
Hence, most of the evaluations need to be conducted under certain assumptions regarding the model's decision process.
The distinction between the notion of plausibility and faithfulness comes from what the assumption on the decision process is.

\textbf{Plausibility} assumes that humans or certain human annotations can convey good desiderata for what important features are for certain model decisions, and that good interpretation should align with these desiderata.
This aligns with certain utility-based views for interpretability evaluations that involve human judgments~\cite{DBLP:conf/chi/AbdulVWLK18,DBLP:conf/iui/FengB19}, as interpretations are, ultimately, used to help humans to understand the behavior of deep learning models.
% However, the main limitation for such criteria is that these deep networks may not follow the same reasoning process as humans tend to deem plausible, and interpretation that faithfully depict these decision process might be down-weighted.
% Besides, although evaluations for model interpretations should be conducted regardless of the correctness of the model's predictions, it is generally easier to establish plausibility for correct predcitions than for erroneous predictions.

On the other hand, \textbf{faithfulness} assumes that the ground-truth reasoning process should not change when a certain factor of the test condition is changed, and compares the interpretations under these the original and the changed test conditions.
For our investigation, we focus on the second faithfulness assumption in~\citet{DBLP:journals/corr/abs-2004-03685}, which assumes that certain perturbations on the model input should not change the interpretation of the same prediction.
% In some way, plausibility is a special case for faithfulness if we treat human as another model and assume they have the same reasoning process.

We believe that combining insights from both perspectives will give a better idea of how well an interpretation method performs on certain models.


==> source/related.tex <==
\section{Related Work}

% To the best of our knowledge, this is the first work to construct dataset for systematic comparison of various post-hoc interpretability methods in the context of NLP.
In this section, we start by familiarize readers with existing work that applies post-hoc interpretation methods to NLP.
We then move on to introduce prior work that validates interpretability methods, both in the context of natural language processing and computer vision.
We end with other interpretability work in NLP that inspired our approach.

% Although only vanilla saliency method was investigated, they were able to show that saliency method uncovers interesting insights about how neural sentiment analysis models work, including the input words where the model most focused on and the way semantic transition is handled by the model.
In the NLP context, \citet{li-etal-2016-visualizing} used the "vanilla" saliency method to probe the decision mechanism of several NLP models and is the first NLP work adopting this interpretation methodology as we are aware of.
Since then, \citet{aubakirova-bansal-2016-interpreting,ding-etal-2017-visualizing,arras-etal-2016-explaining,arras-etal-2017-explaining,mudrakarta-etal-2018-model,ding-etal-2019-saliency} all respectively applies saliency methods to their own tasks of interest and uncovered some useful insights that advanced the understanding for these models, while \citet{DBLP:conf/iclr/MurdochLY18} relied on saliency method as ground truth for analyzing the quality of attention as model interpretation.
Besides, NLP-specific post-hoc interpretation methods have been proposed.
For example, \citet{DBLP:journals/corr/LiMJ16a} proposed \textit{representation erasure} method, which evaluates the saliency of a feature by measuring the change in the output score when the feature is zeroed out.
\citet{DBLP:conf/iclr/MurdochLY18} proposed \textit{context decomposition}, a model-specific saliency method for LSTM, which is further generalized by \citet{jumelet-etal-2019-analysing}.
% We will not elaborate each of them due to space constraints.
As mentioned above, a lot of work in this area builds their conclusion upon the assumption that interpretations obtained from post-interpretation method are always correct.
Even sometimes attested, the evidence for the validity of these methods are largely qualitative.
% Spiritually most similar to this paper, \citet{ding-etal-2019-saliency} quantitatively discussed the ability of several different post-hoc interpretation methods to uncover word alignment from neural machine translation models.
% However, the task of word alignment is an inherently ambiguous one even for humans, and hence is not suitable for evaluations of model interpretations.

% While a significant portion of existing work on interpretability relies solely on qualitative evaluation to determine their effectiveness, there are still studies that performed quantitative analysis.
% The most immediate counterpart of our work is quantitative evaluations of saliency as a metric for the object detection or image segmentation problem in computer vision \cite{DBLP:journals/corr/SimonyanVZ13,DBLP:conf/cvpr/JiangWYWZL13,DBLP:conf/cvpr/LiY15,DBLP:journals/corr/PanWJ15,DBLP:conf/cvpr/OhBKAFS17}, which aims to identify the region containing the most salient object in the image from the background.
In computer vision, the evaluation of post-hoc interpretation methods is conducted by comparing pixel-level post-hoc interpretations with human-annotated ground truth and measuring the area under (precision-recall) curve (AUC) \cite{DBLP:journals/corr/SimonyanVZ13,DBLP:conf/cvpr/JiangWYWZL13,DBLP:conf/cvpr/LiY15,DBLP:journals/corr/PanWJ15,DBLP:conf/cvpr/OhBKAFS17}, on datasets such as PASCAL VOC dataset \cite{pascal-voc-2006}, MSRA dataset \cite{DBLP:conf/cvpr/LiuSZTS07}, and ILSVRC challenge dataset \cite{DBLP:journals/ijcv/RussakovskyDSKS15}.
Extending such evaluation paradigm to NLP, however, is not straight-forward because of the ambiguous and compositional nature of natural language, to the extent that it is often hard even for humans to point out part of the input that is responsible for the model prediction.
To tackle such challenge, \citet{poerner-etal-2018-evaluating,arras-etal-2019-evaluating} individually proposed different frameworks for constructing benchmark tests with clear ground-truth.
They then both conducted analysis on various post-hoc interpretation methods with single-layer recurrent models and concluded methods like DeepLift~\cite{DBLP:conf/icml/ShrikumarGK17}, Layer-wise Relevance Propagation~\cite[LRP][]{bach2015pixel} and Integrated Gradients~\cite{DBLP:conf/icml/SundararajanTY17} with specific composition scheme generate most reliable interpretations.

% There is also work that quantitatively examines the infidelity and sensitiveness of such visual interpretations \cite{DBLP:journals/corr/abs-1901-09392}.
% Apart from that, while mostly constrained to qualitative analysis, \citet{DBLP:conf/nips/AdebayoGMGHK18} proposed sanity checks for saliency methods in the context of compter vision.
% Finally, outside the domain of computer vision, several pieces of work also conduct quantitative human-in-the-loop evaluations.
% For example, \cite{DBLP:journals/corr/abs-1802-00682} conducted human evaluations for various cognitive properties on two hand-crafted, synthetic decision-making task. \cite{DBLP:conf/iui/FengB19} evaluated elastic-search-based interpretation for question answering models by measuring whether these interpretations imporve human performance in Quizbowl.
% Our goal is to provide researchers in the NLP/ML community a NLP counterpart of these computer vision datasets.

Aside from post-hoc interpretability, another important branch of interpretability studies in NLP is targeted evaluations for language models with regard to specific lexical agreements \cite{gulordava-etal-2018-colorless,marvin-linzen-2018-targeted,linzen-etal-2016-assessing}.
Similar targeted evaluations have also been performed for neural machine translation \cite{muller-etal-2018-large,sennrich-2017-grammatical} and coreference resolution \cite{zhao-etal-2018-gender}.
Besides, our benchmarking approach is also inspired by the linguistic probing study of natural language presentations, including contextulized word embeddings \cite{DBLP:conf/acl/TenneyDP19,DBLP:conf/iclr/TenneyXCWPMKDBD19,kim-etal-2019-probing}, sentence embeddings \cite{conneau-etal-2018-cram,DBLP:conf/iclr/AdiKBLG17} and intermediate layers of certain network architecture \cite{shi-etal-2016-string}.
We show in this work that post-hoc interpretations of deep learning models could serve as a good complement for these forms of analysis.


